Robust Neural Networks inspired by Strong Stability Preserving Runge-Kutta methods

Deep neural networks have achieved state-of-the-art performance in a variety of fields. Recent works observe that a class of widely used neural networks can be viewed as the Euler method of numerical discretization. From the numerical discretization perspective, Strong Stability Preserving (SSP) methods are more advanced techniques than the explicit Euler method that produce both accurate and stable solutions. Motivated by the SSP property and a generalized Runge-Kutta method, we propose Strong Stability Preserving networks (SSP networks) which improve robustness against adversarial attacks. We empirically demonstrate that the proposed networks improve the robustness against adversarial examples without any defensive methods. Further, the SSP networks are complementary with a state-of-the-art adversarial training scheme. Lastly, our experiments show that SSP networks suppress the blow-up of adversarial perturbations. Our results open up a way to study robust architectures of neural networks leveraging rich knowledge from numerical discretization literature.

==> figures/resnet_de.tex <==
\begin{figure}
    \centering
    \includegraphics[scale=0.2]{figures/resnet_de.png}
    \caption{
    % ResNet~\cite{he2016identity} as an explicit Euler discretization of numerical integration. Left: One residual block (\textit{ResBlock}). Right: Schematic of the part of the ResNet.
    ResNet~\cite{he2016identity} as an explicit Euler discretization.
    Left: One residual block (\textit{ResBlock}). Right: Schematic of the part of the ResNet.
    }
    \label{fig:resnet_de}
\end{figure}

==> figures/ssp_block_schematic.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{figures/sspblock_schematic.png}
    \caption{Block form}
    \label{fig:ssp_block_schematic}
\end{figure}

==> tables/experimental_description.tex <==
\begin{table}[t]
\centering
\begin{tabular}{c|c|c}
\toprule
Arguments   & Training  & Evaluation    \\
\midrule
$\epsilon$  & 8 & 2,4,8 \\
$alpha$     & 2 &   2   \\
\# of iterations    & 7,12  & 7,12,20   \\
\bottomrule
\end{tabular}
\caption{Experimental Details}
\label{tab:description}
\end{table}

% Need to delete!

==> tables/result_fmnist.tex <==
\begin{table}[t]
    \centering
    % \resizebox{\columnwidth}{!}{
    \begin{tabular}{c|c|c|c}
        \toprule
        Model & Clean & FGSM & PGD$_{20}$ \\
        \midrule\midrule
        ResNet & 0.9090 & 0.8562    & 0.8179 \\
        SSP-2 & 0.9132  & 0.8591    & 0.8252 \\
        SSP-3 & 0.9110  & \textbf{0.8639}    & \textbf{0.8295} \\
        SSP-adap & 0.9098    & 0.8621    & 0.8264
        \bottomrule
    \end{tabular}
    \caption{Result on Fashion MNIST. 20 blocks, groupnorm, train with 0.1 / 0.02 * 10, pgd eval with 0.1 / 0.01 * 20\textbf{}}
    \label{tab:fmnist}
\end{table}

==> tables/ssp_algorithm.tex <==
\begin{algorithm}[t]
\label{alg:ssp2}
%\hspace*{\algorithmicindent} \textbf{Input: }{ddd}	\\
\textbf{Input: }{Input Feature $x(t_k)$, residual block \textit{ResBlock}} \\
\textbf{Output: }{Output Feature $x(t_{k+1})$}
\begin{algorithmic}[1]
\State $x(t_{k+\frac{1}{2}})=\textit{ResBlock}(x(t_k))$
\State $x(t_{k+1})=\frac{1}{2}x(t_k)+\frac{1}{2}\textit{ResBlock}(x(t_{k+\frac{1}{2}}))$
% \While{\textbf{not converge}}
% \For{$(U^i,C^j)$ \textbf{in} $(\mathcal{U,C})$}
% \State Embed user $e_u^{i} \gets U^i$
% \State Initialize $h_0^{j}, c_0^{j}$ as $\textbf{zero}$.
% \For{$V_k^{j}$ \textbf{in} $C^j$}
% \State Embed title $p_k^{j} \gets \mathrm{CharConv}(P_k^{j})$
% \State Embed category $q_k^{j} \gets Q_k^{j}$
% \State Concatenate $p_k^j$ and $q_k^j$, $r_k^{j}=[p_k^{j};q_k^{j}]$
% \State Compute $h_k^{j} = \mathrm{LSTM}(r_k^{j},h_{k-1}^{j},c_{k-1}^{j})$
% \EndFor
% \State Embed channel $e_c^{j} \gets h_{n_j}^{j}$
% \State Compute $\hat{y}_{ij} = \sigma({e_u^{i}} \cdot e_c^{j})$
% \EndFor
% \State Compute loss $\boldsymbol{\mathcal{L}}(\boldsymbol{\theta})$
% \State Gradient descent $\boldsymbol{\theta} := \boldsymbol{\theta} - \epsilon \nabla_{\boldsymbol{\theta}} \boldsymbol{L}(\boldsymbol{\theta})$
% \EndWhile
\end{algorithmic}
\caption{SSP2 block}
\end{algorithm}

==> tables/standard_result.tex <==
% \begin{table}[t]
% \centering
% \begin{tabular}{c|c|c||c|c}
% \toprule
% Training  & Iterations & Model & Accuracy & Gain \\
% \midrule
% \multirow{3}{*}{Standard} & \multirow{3}{*}{-} & res & 0.9259 & - \\
%  & & ssp2 & 0.9226 & -0.0033 \\
%  & & ssp3 & 0.9276 & 0.0017 \\
% \midrule
% \multirow{3}{*}{PGD} & \multirow{3}{*}{7} & res & 0.8357 & - \\
%  & & ssp2 & 0.8257 & -0.1000 \\
%  & & ssp3 & 0.8376 & 0.0019 \\
% \midrule
% \multirow{3}{*}{PGD} & \multirow{3}{*}{12} & res & 0.8010 & - \\
%  & & ssp2 & 0.7899 & -0.1011 \\
%  & & ssp3 & 0.7966 & -0.0044 \\
% \bottomrule
% \end{tabular}
% \caption{Accuracy on clean samples}
% \label{tab:result_standard}
% \end{table}


\begin{table}[t]
\centering
\begin{tabular}{c|c||c}
\toprule
\# of blocks & Model & Accuracy \\
\midrule
\multirow{3}{*}{6} & res & 0.9259 \\
 & ssp2 & 0.9226 \\
 & ssp3 & 0.9276 \\
\midrule
\multirow{3}{*}{10} & res & 0.9318 \\
 & ssp2 & 0.9267 \\
 & ssp3 & 0.9358 \\
\bottomrule
\end{tabular}
\caption{Accuracy on clean samples}
\label{tab:result_standard}
\end{table}
